Refining Language Models with Compositional Explanations

Pre-trained language models have been successful on text classification tasks, but are prone to learning spurious correlations from biased datasets, and are thus vulnerable when making inferences in a new domain. Prior work reveals such spurious patterns via post-hoc explanation algorithms which compute the importance of input features. Further, the model is regularized to align the importance scores with human knowledge, so that the unintended model behaviors are eliminated. However, such a regularization technique lacks flexibility and coverage, since only importance scores towards a pre-defined list of features are adjusted, while more complex human knowledge such as feature interaction and pattern generalization can hardly be incorporated. In this work, we propose to refine a learned language model for a target domain by collecting human-provided compositional explanations regarding observed biases. By parsing these explanations into executable logic rules, the human-specified refinement advice from a small set of explanations can be generalized to more training examples. We additionally introduce a regularization term allowing adjustments for both importance and interaction of features to better rectify model behavior. We demonstrate the effectiveness of the proposed approach on two text classification tasks by showing improved performance in target domain as well as improved model fairness after refinement.

==> chaps/3-problem.tex <==
\subsection{Problem Formulation}
\label{sec:overview}
\vspace{-0.1cm}

% \xiang{Sec 3.1 should be only about definition, goal, and scope (see below) + discussion/comparison with closely related tasks/problem settings + measurement of success/evaluation (at a high level)}



We consider adapting a text classification model $f_S$ trained in a source domain $S$ (\textit{e.g.}, a sentiment classifier trained with news articles) to a new target domain $T$ (\textit{e.g.}, tweets) during a \textit{model refinement} stage. 
We focus on a challenging setting \cite{} where the upstream labeled data $\mathcal{D}_S$ is not available (\textit{e.g.}, due to privacy constraints~\cite{}, or access restriction~\cite{}) but unlabeled data in the target domain ($\mathcal{D}_{T}^{train}$) are accessible, during model refinement.
This setting also reflects the common practice nowadays, as users may download trained models from public model repositories and look to deploy the model to their own data.

We report performance on source data ($\mathcal{D}_S^{test}$) and target data ($\mathcal{D}_T^{test}$) as the measurement of success. We expect the target performance to be improved, while the source performance to be maximally retained, after model refinement. In addition, a refined model should no longer rely on spurious patterns (e.g., being over-sensitive to group identifiers for hate speech detection). Therefore, we report False Positive Rate Difference (FPRD)~\cite{dixon2018measuring}, a fairness metric, for hate speech detection tasks.

% Our problem setting is different from a typical domain adaptation setting, where $\mathcal{D}_S$ is available when making model update~\cite{}. 
% \xiang{expand on comparison with other relevant settings like ``model transfer".}
% Also, the source domain data $\mathcal{D}_S$ may be inaccessible due to privacy concerns. 
% \qinyuan{I rewrote a bit. please help check if things are correct. Do we need more detailed notations? (e.g. $f_S: X \rightarrow Y$ where $X$ is the space of input sentences, $Y$ is the label space, etc.)} 


% \xiang{describe some formal details on the evaluation in a short paragraph -- i.e., how do you measure the success.}


% We consider the setting where a text classification model $f_S$ is first trained on an upstream dataset $\mathcal{D}_S$ from source domain $S$, and is evaluated on a target domain $T$ (see Fig.~\ref{fig:problem_settings}). 
%\xiang{clarify that $\mathcal{D}_S$ may not be available due to reasons like privacy constraint or so.} 
% The classification model takes a sentence $s_i$ as input, and outputs a label $c'_i$ as prediction.
% Considering possible privacy constraints in real application scenario, we assume not to have access to $\mathcal{D}_S$, and only use unlabeled target domain data $\mathcal{D}_T$ in our framework.
%Here, $\mathcal{D}_T$ denotes unlabeled target domain data.
% and is splitted into $\mathcal{D}_T^{train}$, $\mathcal{D}_T^{val}$ and $\mathcal{D}_T^{test}$. 
% \xiang{I don't think we should assume the split are available for the setting. In exp section you can say that we have held-out val/test sets for evaluation purpose.}
% We assume we have access to the labels of $\mathcal{D}^{val}_T$ for the purpose of validating the source model $f_S$ during refinement. Our goal is to improve the refined model's performance on $\mathcal{D}_T^{test}$.
% \xiang{this part and Fig.3 need update because it caused confusion to reviewers. }
% As discussed in Sec.\ref{sec:related}, we apply the setting of sequential transfer learning but aim at obtaining the target model on the same task.
% \xiang{we should have some discussion to draw relationships to traditional learning settings like MTL, transfer leanring, etc; so people can see the commonality and differences, and know where to position our problem setting.}
% \huihan{Discussed in Sec.2.}

%\input{fig_floats/prob_set}
% To provide visualized heat-maps for annotators, we apply the source model $f_S$ to target data $\mathcal{D}_T$ together with an existing post-hoc explanation algorithm $\mathbf{A}$ during prediction. For a sentence, $\mathbf{A}$ will produce an attribution score $\phi_p$ for each word $p$ and we will compute an interaction score $\varphi_{p,q}$ for each word pair $p$ and $q$ based on their attribution scores.

\textbf{Approach Overview.}
% \qinyuan{under construction; working on the notations}
% \xiang{smooth out transition here.}
Our proposed framework has three major steps: 
(1) asking human annotators to check the model's predictions on unlabeled instances, identify the spurious predictions, and write compositional explanations offering suggestions to refine the model;
% collecting and processing human compositional explanations for a model's spurious predictions; 
(2) generalize the collected 
selecting unlabeled instances that matches the descriptions of the explanations; 
% (2) matching explanations with unlabeled instances and 
(3) regularizing the source model $f_S$ with selected unlabeled instances. 
%As a preliminary step, we apply the source model $f_S$ to $\mathcal{D}_T$ together with a post-hoc explanation algorithm $\mathbf{A}$ during prediction. For a sentence, the algorithm $\mathbf{A}$ will produce an attribution score $\phi_p$ for each word $p$ and an interaction score $\varphi_{p,q}$ for each word pair $p$ and $q$.
\xiang{note: variable at the instance level should be uncap like $x_i$ for the $i$ instance, such as explanation, unlabeled data instance, etc.}
In the first step, we first use the source model $f_S$ to make predictions on a small set of unlabeled instances sampled from $\mathcal{D}_S$. We then show the predictions and their hierarchical heat-maps to the annotators (see Fig.~\ref{fig:heatmap}). If the annotator identifies a spurious pattern in the heat-map for instance $I$, a compositional explanation $d$ describing the pattern and their suggestions to refine the model will be provided. In this case, we refer to $I$ as the reference instance for an explanation $d$. 
% Every explanation is based on one instance from $\mathcal{D}_T$, which we refer to as the reference instance $I_{ref}$ that accompanies the explanation.
We then parse every explanation $d$ to $B\rightarrow H$ in the form of first-order logic (FOL) rules, in which B refers to the spurious patterns and H represents human advice on how to adjust attribution/interaction scores of features (\emph{i.e.}, regularization advice).
We denote the collection of explanations as $\mathcal{E}=\{e=(I_{ref}, B, H)\}$. 
In the second step, we design a matching algorithm $\mathbf{G}$ to match every $e_i$ in $\mathcal{E}$ with other instances from $\mathcal{D}_T$.
If an instance is matched with $e_i$, it is supposed to be structurally or semantically similar to $I_{ref, i}$ (\emph{i.e.}, similar spurious pattern described in $B$).
The outputs of $\mathbf{G}$ are denoted as $\mathcal{D}^{match}_T=\{(I, c, r, z)\}$, where $I$ is the input sentence, $c$ is a noisy label, $r$ is the regularization advice, $z$ is a confidence score of matching. 
Finally, we update the model $f_S$ with $\mathcal{D}^{match}_T$ and obtain a refined model $f_T$. Fig.~\ref{fig:framework} illustrates the overview of our framework. 




% We visualize attribution and interaction scores through a hierarchical heat-map and ask annotators to examine those heat-maps of incorrect predictions ($\mathcal{D}_e$) to solicit a small set of regularization rules $\mathcal{D}_R$ (\emph{i.e.} natural language compositional explanations). 
%In the second step, we parse all explanations in $\mathcal{E}$ into first-order logic rules, and then design a matching algorithm $\mathbf{G}$ to match other instances from $\mathcal{D}_T$.
% Then we apply our soft matching algorithm $\mathcal{G}$ to generalize the rules to a large number of unlabeled instances from target domain, which will serve as the training set $\mathcal{D}^{train}_T=\{(s, c, r, z)\}$, where $c$ is noisy label for the sentence $s$, $r$ is the regularization advice parsed from the rule, $z$ is a confidence score given by $\mathcal{G}$. Finally we fine-tune the existing model with $\mathcal{D}^{train}_T$ and re-evaluate the refined model $f_T$ to see the performance improvement. Fig.~\ref{fig:framework} illustrates the overview of our framework. 
%During the regularization stage, we use $\mathcal{D}^{val}_T$ as validation set to conduct early stopping.




==> chaps/x-checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See page 11.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Appendix~\ref{app:reproduce}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{app:reproduce}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{app:reproduce}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Open-source.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Appendix.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Appendix.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig_floats/exp_num.tex <==
%\begin{figure}[t]
%\vspace{0.2cm}
%    \centering
%    \includegraphics[width=0.42\textwidth]{figure/explanation-numbers.pdf}
    %\vspace{0.2cm}
%    \caption{\small \textbf{Performance on GHC refined from Stormfront using different number of explanations.} More explanations introduce more diverse human knowledge and thus lead to better performance after model refinement.
%    }% \xiang{1) explain the dash line; 2) enlarge x/y-axis font size; reudce height of the fig.}}
%    \label{fig:explanation_number}
%    \vspace{-0.1cm}
%\end{figure}

\begin{figure}[h]
\vspace{0.1cm}
\begin{minipage}{0.48\textwidth}
  \centerline{\includegraphics[width=0.9\textwidth]{figure/explanation-numbers.pdf}}
  \vspace{-0.1cm}
  \centerline{\small (a) StormFront to GHC}
\end{minipage}
%\begin{minipage}{0.15\textwidth}
%  \centerline{\includegraphics[width=2.5cm]{figure/reg_strength_hateval.png}}
%  \centerline{\tiny (b) HatEval to GHC}
%\end{minipage}
\begin{minipage}{0.48\textwidth}
  \centerline{\includegraphics[width=0.9\textwidth]{figure/explanation-numbers-hateval.pdf}}
  \vspace{-0.1cm}
  \centerline{\small (b) HatEval to GHC}
\end{minipage}
  \vspace{-0.1cm}
\caption{\small \textbf{Performance on GHC refined from Stormfront and HatEval using different number of explanations.} More explanations introduce more diverse human knowledge and thus lead to better performance after model refinement.
\xiang{can keep one dataset and move the other to appendix; with a pointer in exp writing (say ``similar pattern in the other dataset").}
}
\label{fig:explanation_number}
\vspace{-0.4cm}
\end{figure}


==> fig_floats/exp_num_hateval.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\vspace{-0.2cm}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/explanation-numbers-hateval.pdf}
    \vspace{-0.5cm}
    \caption{\small \textbf{Performance on GHC refined from HatEval using different number of explanations.} %More explanations introduce more diverse human knowledge and thus lead to better performance after model refinement.
    }
    
    \label{fig:exp_num_hateval}
    \vspace{-0.2cm}
\end{wrapfigure}

==> fig_floats/exp_num_stormfront.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\vspace{-0.2cm}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/explanation-numbers.pdf}
    % \vspace{-0.5cm}
    \caption{\small \textbf{Different Explanation Numbers}}
    
    \label{fig:exp_num_stormfront}
    %\vspace{-0.6cm}
\end{wrapfigure}

==> fig_floats/hard_soft.tex <==
\begin{wrapfigure}{R}{0.36\textwidth}
    % \vspace*{-0.5cm}
    \centering
    \includegraphics[width=0.35\textwidth]{figure/hard-soft.png}
    \vspace{-0.2cm}
    \caption{\small \textbf{Hard and soft matching with regularization.}
    % \xiang{needs update}
    }
    \label{fig:hard_soft}
    % \vspace*{-0.4cm}
\end{wrapfigure}

==> fig_floats/module.tex <==
\begin{wrapfigure}{R}{0.45\textwidth}
    \vspace*{-0.3cm}
    \centering
    \includegraphics[width=0.45\textwidth]{figure/module.png}
    \vspace{-0.5cm}
    \caption{\small \textbf{Examples for FILL/FIND modules.} 
    %Fill module can capture structure similarities, such as named entity type, part-of-speech tag, etc. FIND module can detect synonyms of $p_{ref}$.
    }
    \label{fig:module}
    \vspace*{-0.4cm}
\end{wrapfigure}

==> fig_floats/neg_samp.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\vspace{-0.2cm}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/neg-ratio.pdf}
    \vspace{-0.5cm}
    \caption{\small \textbf{Sensitivity study on different negative samplings. \xiang{can move the detailed discussion to appendix; and in exp writing briefly summarize the observations (e.g., sensitive or not)}
}
    %The model is not quite sensitive to different sampling numbers and different samplings of the same amount.
    }
    \label{fig:sensitivity_negative_sampling}
    \vspace{-0.6cm}
\end{wrapfigure}

==> fig_floats/prob_set.tex <==
\begin{wrapfigure}{R}{0.49\textwidth}
    \vspace*{-0.3cm}
    \centering
    \includegraphics[width=0.45\textwidth]{figure/setting_updated.png}
    \vspace{-0.2cm}
    \caption{\small \textbf{Illustration of the problem setting for model refinement with compositional explanation via regularization technique.}
    % \xiang{needs update}
    }
    \label{fig:problem_settings}
    \vspace*{-0.3cm}
\end{wrapfigure}

==> floats/tab_case_study.tex <==
% \begin{table}[h]
% \centering
% \caption{Matched rule for Figure \ref{fig:case_study}.}
% \vskip 0.1in
% \scalebox{0.82}{
% \begin{tabular}{p{10cm}}
% \toprule
%     \makecell[l{p{10cm}}]{
%     % \textbf{\underline{Compositional Explanation}}\\
%     % \textbf{Label:} Hateful\\
%     \small{
%     \textbf{Rule Body}: X is ``\textcolor{Blue}{\textbf{\textit{dumb}}}". Y is a hateful word. X is immediately before Y.}\\ 
%     \small{
%     \textbf{Rule Head}: Attribution score of X should be increased. Attribution score of Y should be increased. The interaction score of X and Y should be increased.}}  \\
%     % \midrule
%     % \makecell[l{p{10cm}}]{\textbf{\underline{Notes}}\\
%     % \textbf{Faggot} is a hateful word. }\\
% \bottomrule
% \end{tabular}
% }
% \vskip -0.2in
% \label{tab:case_study_rule}
% \end{table}

==> floats/tab_explanation_parsing.tex <==
\begin{table}[h]
    \centering
    \caption{\small\textbf{An example of explanation parsing.} Human annotators provide compositional explanations in natural language. The explanations are parsed as first-order logic rules.
    %\xiang{can move to appendix given we have similar info in Fig. 2?}
    }
    \scalebox{0.8}{
    \begin{tabular}{p{10cm}}
    \toprule
        \makecell[l{p{10cm}}]{\textbf{\underline{Compositional Explanation}}\\
        \textbf{Instance:} \textcolor{Blue}{\textbf{\textit{Sweden}}} has been proved to be a \textcolor{BrickRed}{\textbf{\textit{failure}}}.\\
        \textbf{Natural Language Explanation}: \\
        X is ``\textcolor{Blue}{\textbf{\textit{Sweden}}}". Y is ``\textcolor{BrickRed}{\textbf{\textit{failure}}}". X is a country. Y is negative. X is less than 3 dependency steps from Y. Therefore, attribution of X should be decreased, attribution of Y should be increased, and interaction of X and Y should be increased.}  \\
        \textbf{First-Order Logic Rule}: \\
        @Is(X,country) $\wedge$ @Is(Y,negative) $\wedge$ @DependencyLessThan(X,Y,3) $\rightarrow$ DecreaseAttribution(X) $\wedge$ IncreaseAttribution(Y)$\wedge$ IncreaseInteraction(X, Y)\\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-0.2cm}
    
    \label{tab:explanation_parsing}
\end{table}

==> floats/tab_general.tex <==
\begin{wraptable}{R}{0.6\textwidth}
\centering
\begin{tabular}{c|c|c|c}
\toprule
    Dataset Pairs & threshold & coverage & precision \\ \midrule
    HatEval$\rightarrow$GHC & 0.55 & 370 & 0.692 \\ \midrule
    Stormfront$\rightarrow$GHC & 0.7 &  & \\ \midrule
    Amazon$\rightarrow$SST-2 & 0.6 & 1737 & 0.917 \\ \midrule

\end{tabular}
\label{tab:general_eval}
\end{wraptable}

==> floats/tab_ghc.tex <==
\begin{table*}[t]
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lccccr}
\toprule
%Method  & F1 & NYT Accuracy & IPTT F1 & IPTT FPR \\
Method  & F1 & IPTT F1 & IPTT FPR \\
\midrule
%Original model from Stormfront  & $0.421\pm0.015$ & $0.830\pm0.056$ & $0.529\pm0.099$ & $0.013\pm0.006$\\
Original model from Stormfront  & $0.421\pm0.015$ & $0.529\pm0.099$ & $0.013\pm0.006$\\
% Only Reg: Hard match reg. with IG & $0.439 \pm 0.001$  & $0.793 \pm 0.006 $  & $0.425 \pm 0.012 $ & $ 0.005 \pm 0.000 $ \\ % 0.1, 5e-6
%Only Reg: Hard match reg. with IG & $0.437 \pm 0.004$  & $0.787 \pm 0.012$  & $0.433 \pm 0.016$  & $0.006 \pm 0.001 $ \\ % 0.1, 5e-6
Only Reg: Hard match reg. with IG & $0.437 \pm 0.004$ & $0.433 \pm 0.016$  & $0.006 \pm 0.001 $ \\ % 0.1, 5e-6
%Only Reg: Hard match reg. with SOC &  $0.443\pm0.007$ & $0.881\pm0.029$ &$0.559\pm0.102$ &$0.007\pm0.005$\\
Only Reg: Hard match reg. with SOC &  $0.443\pm0.007$ &$0.559\pm0.102$ &$0.007\pm0.005$\\
%Only Reg: Soft match reg. with IG & $0.443 \pm 0.011$ & $ 0.842 \pm 0.061 $  & $ 0.330 \pm 0.137 $ & $ 0.003 \pm 0.002 $ \\
Only Reg: Soft match reg. with IG & $0.443 \pm 0.011$ & $ 0.330 \pm 0.137 $ & $ 0.003 \pm 0.002 $ \\
%Only Reg: Soft match reg. with SOC & $0.457\pm0.014$ & $0.837\pm0.033$ & $0.558\pm0.246$ & $0.006\pm0.009$\\
Only Reg: Soft match reg. with SOC & $0.457\pm0.014$ & $0.558\pm0.246$ & $0.006\pm0.009$\\
\midrule
%Only Labels: Hard match label(+Neg Samples) & $0.495\pm0.009$ & $0.504\pm0.040$ &$0.559\pm0.102$ & $0.007\pm0.005$\\
Only Labels: Hard match label(+Neg Samples) & $0.495\pm0.009$ &$0.559\pm0.102$ & $0.007\pm0.005$\\
%\makecell[l{p{6cm}}]{Reg.+Labels: Hard match label(+Neg Samples) \\ \quad \quad \quad \quad \quad \quad + Soft match reg. with IG}  & $0.457 \pm 0.002 $ & $ 0.698 \pm 0.042 $ & $ 0.612 \pm 0.280  $ & $ 0.012 \pm 0.003 $ \\ % 0.02, 1e-4
\makecell[l]{Reg.+Labels: Hard match label(+Neg Samples) + Soft match reg. with IG}  & \textcolor{red}{$0.457 \pm 0.002 $} & $ 0.612 \pm 0.280  $ & $ 0.012 \pm 0.003 $ \\ % 0.02, 1e-4
%\makecell[l{p{6cm}}]{Reg.+Labels: Hard match label(+Neg Samples) , nointer\\ \quad \quad \quad \quad \quad \quad + Soft match reg. with IG} & 0.465 \pm 0.022 &  & & \\ % 0.02, 7e-5
%\makecell[l{p{6cm}}]{Reg.+Labels: Hard match label(+Neg Samples) \\ \quad \quad \quad \quad \quad \quad + Soft match reg. with SOC} & $0.494\pm0.020$ &$0.703\pm0.081$ &$0.716\pm0.125$ &$0.008\pm0.004$ \\
\makecell[l]{Reg.+Labels: Hard match label(+Neg Samples) + Soft match reg. with SOC} & \color{red}$0.494\pm0.020$ &$0.716\pm0.125$ &$0.008\pm0.004$ \\
%Fine-tune with GHC (Upper bound) &$0.529\pm0.010$ &$0.744\pm0.094$ &$0.593\pm0.092$ &$0.040\pm0.039$ \\
Fine-tune with GHC (Upper bound) &$0.529\pm0.010$ &$0.593\pm0.092$ &$0.040\pm0.039$ \\
\midrule
%Original model from HatEval & $0.295\pm0.025$ &$0.982\pm0.015$ &$0.332\pm0.153$ &$0.053\pm0.049$\\
Original model from HatEval & $0.295\pm0.025$ &$0.332\pm0.153$ &$0.053\pm0.049$\\
%Hard match reg. with IG, inter & $0.339\pm0.011$ &  & & \\ % 0.1, 2e-5
%Only Reg: Hard match reg. with IG & $0.334\pm0.004$ & $0.976 \pm 0.021$ & $0.486 \pm 0.061$ & $ 0.137 \pm 0.053 $ \\ % 0.1, 2e-5
Only Reg: Hard match reg. with IG & $0.334\pm0.004$ & $0.486 \pm 0.061$ & $ 0.137 \pm 0.053 $ \\ % 0.1, 2e-5
%Only Reg: Hard match reg. with SOC & $0.394\pm0.005$ &$0.979\pm0.029$ &$0.706\pm0.135$ &$0.025\pm0.020$\\
Only Reg: Hard match reg. with SOC & $0.394\pm0.005$ &$0.706\pm0.135$ &$0.025\pm0.020$\\
%Only Reg: Soft match reg. with IG, inter & $0.347 \pm 0.008$ & $0.983 \pm 0.016$  & $0.429 \pm 0.059 $ & $ 0.103 \pm 0.031 $ \\ % 0.02, 2e-5
Only Reg: Soft match reg. with IG & $0.347 \pm 0.008$ & $0.429 \pm 0.059 $ & $ 0.103 \pm 0.031 $ \\ % 0.02, 2e-5
%Only Reg: Soft match reg. with IG, nointer & $0.339 \pm 0.014 $ & & & \\ % 0.01, 1e-5
%Only Reg: Soft match reg. with SOC & $0.399\pm0.021$ &$0.981\pm0.015$ &$0.665\pm0.119$ &$0.028\pm0.017$\\
Only Reg: Soft match reg. with SOC & $0.399\pm0.021$ &$0.665\pm0.119$ &$0.028\pm0.017$\\
\midrule
%Only Labels: Hard match label & $0.485\pm0.001$ &$0.927\pm0.024$ &$0.706\pm0.135$ &$0.025\pm0.020$ \\
Only Labels: Hard match label & $0.485\pm0.001$ &$0.706\pm0.135$ &$0.025\pm0.020$ \\
% \makecell[l]{Reg.+Labels: Hard match label(+Neg Samples) + Soft match reg. with IG} & & & \\
%\makecell[l{p{6cm}}]{Reg.+Labels: Hard match label(+Neg Samples) \\ \quad \quad \quad \quad \quad \quad + Soft match reg. with SOC} & $0.464\pm0.016$ &$0.945\pm0.016$ &$0.806\pm0.014$ &$0.032\pm0.002$ \\ %
\makecell[l]{Reg.+Labels: Hard match label(+Neg Samples) + Soft match reg. with IG} & \textcolor{red}{$0.462\pm0.007$} &$0.678\pm0.149$ &$0.075\pm 0.067$ \\ % 0.02, 1e-4
%\makecell[l]{Reg.+Labels: Hard match label(+Neg Samples) + Soft match reg. with IG} & $0.462\pm0.007$ &$0.806\pm0.014$ &$0.032\pm0.002$ \\ % 0.005, 1e-4, nointer
\makecell[l]{Reg.+Labels: Hard match label(+Neg Samples) + Soft match reg. with SOC} & \color{red}$0.464\pm0.016$ &$0.806\pm0.014$ &$0.032\pm0.002$ \\ %
%Fine-tune with GHC (Upper bound) & $0.515\pm0.009$ &$0.874\pm0.040$ & $0.701\pm0.058$ &$0.184\pm0.020$  \\
Fine-tune with GHC (Upper bound) & $0.515\pm0.009$ & $0.701\pm0.058$ &$0.184\pm0.020$  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\caption{F1 score on Gab Hate Corpus, NYT accuracy and results on Identity Phrase Templates Test Set for different regularization settings on hate speech task.
\xiang{1) show two test sets by columns; 2) do XX.X for F1 (in \%)}
}
\label{ghc-main-table}
\end{table*}



==> floats/tab_hate_nonhate_ghc.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Method  & F1 & IPTT F1 & IPTT FPR\\
\midrule
\makecell[l]{Original model\\from Stormfront} & $0.421\pm0.015$ & $0.529\pm0.099$ & $0.013\pm0.006$\\
Hateful rules & $0.457\pm0.014$ & $0.558\pm0.246$ & $0.006\pm0.009$ \\
Non-hateful rules & $0.434\pm0.004$ & & \\
All rules & $0.450\pm0.008$ &$0.545\pm0.096$ & $0.007\pm0.004$ \\
\midrule
\makecell[l]{Original model\\from HatEval} & $0.295\pm0.025$ &$0.332\pm0.153$ &$0.053\pm0.049$\\
Hateful rules & $0.399\pm0.021$ & $0.665\pm0.119$ &$0.028\pm0.017$ \\
Non-hateful rules & $0.321\pm0.005$ & & \\
All rules & $\pm$ & & \\
\bottomrule
\end{tabular}
}
\vspace{-0.2cm}
\caption{Studying effects of hateful and non-hateful rules on Gab Hate Corpus.}
\label{gab-rules-table}
\end{table}



==> floats/tab_hateval.tex <==
%\begin{table*}[t]
%\caption{F1 score on Gab Hate Corpus, NYT accuracy and results on Identity Phrase Templates Test Set with original model trained on HatEval.}
%\label{hateval-main-table}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{tabular}{lcccr}
%\toprule
%Method  & F1 & NYT Accuracy & IPTT F1 & IPTT FPR\\
%\midrule
%Original model from HatEval & $0.295\pm0.025$ &$0.982\pm0.015$ &$0.332\pm0.153$ &$0.053\pm0.049$\\
%%Hard match reg. with IG, inter & $0.339\pm0.011$ &  & & \\ % 0.1, 2e-5
%Hard match reg. with IG & $0.334\pm0.004$ &  & & \\ % 0.1, 2e-5
%Hard match reg. with SOC & $0.394\pm0.005$ &$0.979\pm0.029$ &$0.706\pm0.135$ &$0.025\pm0.020$\\
%Soft match reg. with IG, inter & $0.347 \pm 0.008$ &  & & \\  0.02, 2e-5
%Soft match reg. with IG & $0.339 \pm 0.014 $ & & & \\ % 0.01, 1e-5
%Soft match reg. with SOC & $0.399\pm0.021$ &$0.981\pm0.015$ &$0.665\pm0.119$ &$0.028\pm0.017$\\
%\midrule
%Hard match label & $0.485\pm0.001$ &$0.927\pm0.024$ &$0.706\pm0.135$ &$0.025\pm0.020$ \\
%Hard match label + Soft match reg. with SOC & $0.464\pm0.016$ &$0.945\pm0.016$ &$0.806\pm0.014$ &$0.032\pm0.002$ \\ %
%Fine-tune with GHC (Upper bound) & $0.515\pm0.009$ &$0.874\pm0.040$ & $0.701\pm0.058$ &$0.184\pm0.020$  \\
%\bottomrule
%\end{tabular}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table*}


==> floats/tab_interaction.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Ablation study on regularizing attribution and interaction.} Both regularizing attribution and interaction scores  yield improvements over the source model.}
\vskip 0.15in
\scalebox{0.85}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Dataset} & \multicolumn{2}{c}{\small\textbf{\begin{tabular}[c]{@{}c@{}}Stormfront$\rightarrow$GHC\end{tabular}}} & \multicolumn{1}{c}{\small\textbf{\begin{tabular}[c]{@{}c@{}}AmazonMusic$\rightarrow$SST-2\end{tabular} }} \\ \midrule
\textbf{Metrics}           & \textbf{\small\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\small\begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} &   \textbf{\small\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} \\ \midrule
\textbf{Source model} & 42.1$\pm$1.5 &  16.0  & 83.5$\pm$2.5  \\
\textbf{reg. with a.} & 44.6$\pm$1.6 &  7.2  & 85.3$\pm$0.1  \\
\textbf{reg. with i.} & 43.2$\pm$0.1 &  8.5  & 85.1$\pm$0.1  \\
% \textbf{reg. with a. \& i.} & \textbf{45.7$\pm$1.4} &  12.6 & 85.2$\pm$0.2  \\
 \bottomrule
\end{tabular}
}
\label{tab:ablation_interaction}
% \vspace{-0.2cm}
\end{table}

==> floats/tab_interaction_ghc.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Method  & F1 & IPTT F1 & IPTT FPR\\
\midrule
\makecell[l]{Original model\\from Stormfront} & $0.421\pm0.015$ & $0.529\pm0.099$ & $0.013\pm0.006$\\
reg. with a. & $0.450\pm0.012$ & $0.531\pm0.052$ & $0.006\pm0.001$\\
reg. with i. & $0.432\pm0.001$ & $0.449\pm0.022$ & $0.006\pm0.001$\\
reg. with a. \& i. & $0.457\pm0.014$ & $0.558\pm0.246$ & $0.006\pm0.009$\\
\midrule
\makecell[l]{Original model\\from HatEval} & $0.295\pm0.025$ &$0.332\pm0.153$ &$0.053\pm0.049$\\
% Soft match reg. importance & $0.361\pm0.011$ & $0.436\pm0.011$ & $0.395\pm0.003$\\
reg. with a. & $0.399\pm0.021$ & $0.665\pm0.119$ &$0.028\pm0.017$ \\
reg. with i. & $0.321\pm0.000$ & & \\
reg. with a. \& i. & \color{red}$0.397\pm0.006$ & $0.495\pm0.027$ & $0.010\pm0.008$ \\
\bottomrule
\end{tabular}
}
\vspace{-0.2cm}

\caption{Studying effects of regularizing importance and interaction on Gab Hate Corpus.}
\label{ghc-interaction-table}
\end{table}


%\begin{table*}[t]
%\vskip 0.15in
%\begin{center}
%\begin{small}

%\end{small}
%\end{center}
%\vskip -0.1in

%\end{table*}

==> floats/tab_interaction_hateval.tex <==
\begin{table*}[t]
\caption{Studying effects of regularizing importance and interaction on Gab Hate Corpus with original model trained on HatEval.}
\label{hat-interaction-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lccccr}
\toprule
Method  & Precision & Recall & F1\\
\midrule
Original model from HatEval\\
% Soft match reg. importance & $0.361\pm0.011$ & $0.436\pm0.011$ & $0.395\pm0.003$\\
Soft match reg. importance & $0.316\pm0.030$ & $0.560\pm0.107$ & $0.399\pm0.021$\\
Soft match reg. interaction & $0.268\pm0.003$ & $0.402\pm0.006$ & $0.321\pm0.000$\\
Soft match reg. importance and interaction & $0.316\pm0.017$ & $0.527\pm0.004$ & $0.395\pm0.013$\\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> floats/tab_interaction_new.tex <==
\begin{table}[h]
\centering
\caption{Studying effects of regularizing attribution and interaction}
\vskip 0.15in
\scalebox{0.8}{
\begin{tabular}{@{}l|cc|c@{}}
\toprule
\textbf{Dataset} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Stormfront\\ $\rightarrow$ GHC\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}AmazonMusic\\ $\rightarrow$ SST-2\end{tabular} }} \\ \midrule
\textbf{Metrics}           & \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} &   \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} \\ \midrule
\textbf{Original Model} & 42.1$\pm$1.5 &  16.0 & 83.5$\pm$2.5  \\
\textbf{reg. with a.} & 44.6$\pm$1.6 &  7.2  & 85.3$\pm$0.1  \\
\textbf{reg. with i.} & 43.2$\pm$0.1 &  8.5  & 85.1$\pm$0.1  \\
\textbf{reg. with a. \& i.} & 43.7$\pm$1.0 &   & 85.2$\pm$0.2  \\
 \bottomrule
\end{tabular}
}
\label{tab:ablation_interaction}
\vspace{-0.2cm}
\end{table}

==> floats/tab_interaction_sst2.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Method  & Precision & Recall & F1\\
\midrule
Original model & $0.902\pm0.032$ & $0.781\pm0.064$ & $0.835\pm0.025$\\
reg. with a. & $0.863\pm0.007$ & $0.843\pm0.008$ & $0.853\pm0.001$\\
reg. with i. & $0.867\pm0.001$ & $0.835\pm0.006$ & $0.851\pm0.003$\\
reg. with a. \& i.  & $0.861\pm0.010$ & $0.843\pm0.006$ & \textcolor{red}{$0.852\pm0.002$}\\
\bottomrule
\end{tabular}
}
\vspace{-0.2cm}
%\vskip 0.15in
%\begin{center}
%\begin{small}

%\end{small}
%\end{center}
%\vskip -0.1in
\caption{Studying effects of regularizing importance and interaction on SST-2.}
\label{sst-interaction-table}
\end{table}


==> floats/tab_lm.tex <==
\begin{table}[h]
\vspace{-0.1cm}
\centering
\caption{\textbf{Refining BERT-Large and RoBERTa-Base.} Results are from the HatEval $\rightarrow$ GHC setting. Our method also effectively improves the source models that are built upon other pre-trained language models.}
\vskip 0.15in
\scalebox{0.75}{
\begin{tabular}{@{}lcccc}
\toprule
\textbf{Language Model} & \multicolumn{2}{c}{\small\textbf{\begin{tabular}[c]{@{}c@{}}BERT-Large\end{tabular}}} & \multicolumn{2}{c}{\small\textbf{\begin{tabular}[c]{@{}c@{}}RoBERTa-Base\end{tabular} }} \\ 
\midrule
\textbf{Metrics}           & \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} &   \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} \\ \midrule
Source model & 31.4$\pm$1.4 & 124.3 & 30.9$\pm$1.9 & 61.6 \\
\midrule
\multicolumn{5}{l}{\hspace{-0.2cm}\textit{With only reg.} \cellcolor{na}}\\\midrule
~~-~Hard reg. with SOC & 33.6$\pm$1.1 & 134.0 & 37.9$\pm$1.5 & 14.2 \\
~~-~Soft reg. with SOC & 35.6$\pm$3.3 & 42.4 & 39.4$\pm$0.5 & 20.6\\
\midrule
\multicolumn{5}{l}{\hspace{-0.2cm}\textit{With reg. \& noisy labels} \cellcolor{na}}\\\midrule
~~-~No reg. & 49.4$\pm$0.8 & 56.7 & 47.8$\pm$0.4 & 244.7 \\
~~-~Soft reg. with SOC & 48.7$\pm$1.5 & 49.5 & 48.1$\pm$1.7 & 126.8 \\\midrule
Upper bound & 52.5$\pm$0.4 & 98.0 & 50.6$\pm$0.4 & 263.2\\
\bottomrule
\end{tabular}
}
\label{tab:lm}
% \vspace{-0.2cm}
\end{table}

==> floats/tab_lstm.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Results for Bi-LSTM.}}
\scalebox{0.65}{
\begin{tabular}{@{}l|ccc|ccc|cc@{}}
\toprule
\textbf{Dataset} & \multicolumn{3}{c|}{\small\textbf{HatEval $\rightarrow$ GHC}} & \multicolumn{3}{c|}{\small\textbf{Stormfront $\rightarrow$ GHC}} & \multicolumn{2}{c}{\small\textbf{AmazonMusic $\rightarrow$ SST-2}} \\ \midrule
\textbf{Metrics}           & 
\textbf{\small\begin{tabular}[c]{@{}c@{}}Source  F1 ($\uparrow$)\end{tabular}} & \textbf{\small\begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} & 
\textbf{\small\begin{tabular}[c]{@{}c@{}}Source F1($\uparrow$)\end{tabular}} &
\textbf{\small\begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} & \textbf{\small\begin{tabular}[c]{@{}c@{}}Source F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} \\ \midrule

Source model (Bi-LSTM) & 60.5$\pm$0.7 & 20.2$\pm$1.2  & 115.2 & 44.7$\pm$2.2 & 26.3$\pm$4.2  & 157.2 & 81.1$\pm$1.5 & 54.0$\pm$5.5 \\ \midrule
\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With only reg.}}\\ \midrule
% ~~- Hard reg. with SOC & 61.2$\pm$0.0 & 23.0$\pm$0.6  & 114.3 & $\pm$ & 27.7$\pm$1.5  & 72.5 & 78.4$\pm$1.7 & 64.1$\pm$0.9 \\
~~- Reg. with SOC& 61.1$\pm$0.1 & 23.0$\pm$0.4  & 69.3 & $\pm$ & 28.5$\pm$0.9  & 18.6 & \textbf{78.5$\pm$0.7} & \textbf{64.9$\pm$1.5}\\ \midrule

\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With reg. \& noisy labels}}\\\midrule
~~- No reg.  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & \textbf{78.9$\pm$0.4} & 61.0$\pm$1.3 \\
~~- Baseline:L2-reg. & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & 78.7$\pm$0.4 & 62.6$\pm$1.1 \\
~~- Baseline:Distillation & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & 78.6$\pm$0.6 & 61.6$\pm$1.3 \\
%~~- Soft reg. with IG &  $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\
~~- Soft reg. with SOC & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & 76.9$\pm$0.5 & \textbf{66.1$\pm$0.6} \\ \midrule

Upper bound & 58.5$\pm$1.7 & 38.5$\pm$1.7  & 124.2 & 42.5$\pm$2.0 & 44.5$\pm$0.2  & 323.3 & 79.2$\pm$0.2 & 81.7$\pm$1.1 \\

\bottomrule
\end{tabular}
}
\end{table}

==> floats/tab_main.tex <==
\begin{table*}[t]
\vspace{-0.1cm}
\centering
\caption{\textbf{Main Results for different regularization settings.} We repoart F1 score on GHC and SST-2 as target domain performance, and FPRD on IPTTS as fairness metric for hate speech task.}
\vskip 0.15in
\scalebox{0.90}{
\begin{tabular}{@{}l|ccc|ccc|cc@{}}
\toprule
\textbf{Dataset} & \multicolumn{3}{c|}{\textbf{Stormfront $\rightarrow$ GHC}} & \multicolumn{3}{c|}{\textbf{Hateval $\rightarrow$ GHC}} & \multicolumn{2}{c}{\textbf{AmazonMusic $\rightarrow$ SST-2}} \\ \midrule
\textbf{Metrics}           & 
\textbf{\begin{tabular}[c]{@{}c@{}}Source\\ F1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Target\\ F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Source\\ F1\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Target\\ F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Source\\ F1 \end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Target\\ F1 ($\uparrow$)\end{tabular}} \\ \midrule
\textbf{Original Model} & 57.2$\pm$0.7 & 42.1$\pm$1.5 &  16.0  & 64.2$\pm$0.3 & 29.5$\pm$2.5  & 115.6 & 91.4$\pm$0.4 &83.5$\pm$2.5  \\ \midrule

\textbf{Only Reg.:}\\
\textbf{Hard reg. with IG} & 55.4$\pm$1.8 & 43.7$\pm$0.2  & 23.3 & 63.2$\pm$0.6  & 34.4$\pm$1.4  &  197.2 & 91.1$\pm$0.0 & 85.2$\pm$0.1  \\ % 0.1, 5e-6 / 0.1, 5e-6
\textbf{Hard reg. with SOC} & 53.2$\pm$1.5 & 44.3$\pm$0.7  & 8.7  & 63.0$\pm$1.1 & 39.4$\pm$0.5  & 43.1 & 91.1$\pm$0.0 & 85.2$\pm$0.3  \\
\textbf{Soft reg. with IG} &55.7$\pm$0.5& 44.3$\pm$1.1  & 23.3 & 63.9$\pm$0.7 &34.7$\pm$0.8  & 170.9 & 91.1$\pm$0.0 & 85.0$\pm$0.2  \\ % 0.1, 7e-6, 0.05, 5e-6
\textbf{Soft reg. with SOC} & 49.9$\pm$3.5 & 45.7$\pm$1.4  & 12.6 & 62.0$\pm$0.3 & 39.9$\pm$2.1  &  50.2  & 91.1$\pm$0.0 & 85.3$\pm$0.1  \\ \midrule

\textbf{With Noisy Labels:}\\
\textbf{No reg.} & 44.3$\pm$2.9 & 49.5$\pm$0.9  & 130.6  & 58.8$\pm$1.0 & 48.5$\pm$0.1  &  144.7  & 90.7$\pm$0.1 & 86.0$\pm$0.6  \\
\textbf{Soft reg. with IG} &51.4$\pm$4.6 & 47.5$\pm$1.1  & 12.76 & 61.9$\pm$0.9 & 48.1$\pm$3.0  & 199.3 & 91.2$\pm$0.1 & 87.0$\pm$3.7  \\ % 0.02, 5e-5 40: 0.02 / 5e-5, 0.005 / 7e-5
\textbf{Soft reg. with SOC} & 50.6$\pm$1.7 & 49.4$\pm$2.0  & 23.3 & 60.8$\pm$1.3 & 46.4$\pm$1.6  &  79.8  & 91.1$\pm$0.2 & 87.3$\pm$0.1  \\ \midrule

\textbf{Upper bound} & 46.9$\pm$2.4 & 52.9$\pm$1.0  & 115.0 & 60.0$\pm$2.3 & 51.5$\pm$0.9  &  333.3  & 90.4$\pm$0.1& 92.9$\pm$0.4  \\

 \bottomrule
\end{tabular}
}

\label{tab:main_results}
\vspace{-0.3cm}
\end{table*}

==> floats/tab_main_all.tex <==


\begin{table*}[t]
% \vspace{-0.1cm}
\centering
\caption{\textbf{Main Results on BERT-Base, BERT-Large and RoBERTa-Base for different regularization settings on three pairs of datasets.} We report F1 scores on source domain and target domain, and FPRD on IPTTS as fairness metric for hate speech task. Best results are \textbf{bold}. 
%Regularization based on both hard- and soft-matching improves the target domain performance of the source model, and also reduces unintended bias.
}
\vspace{-0.2cm}
\scalebox{0.68}{
\begin{tabular}{@{}l|ccc|ccc|cc@{}}
\toprule
\textbf{Dataset} & \multicolumn{3}{c|}{\small\textbf{HatEval $\rightarrow$ GHC}} & \multicolumn{3}{c|}{\small\textbf{Stormfront $\rightarrow$ GHC}} & \multicolumn{2}{c}{\small\textbf{AmazonMusic $\rightarrow$ SST-2}} \\ \midrule
\textbf{Metrics}           & 
\textbf{\small\begin{tabular}[c]{@{}c@{}}Source  F1 ($\uparrow$)\end{tabular}} & \textbf{\small\begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} & 
\textbf{\small\begin{tabular}[c]{@{}c@{}}Source F1($\uparrow$)\end{tabular}} &
\textbf{\small\begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} & \textbf{\small\begin{tabular}[c]{@{}c@{}}Source F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} \\ \midrule



Source model (BERT-b) & 64.2$\pm$0.3 & 29.5$\pm$2.5  & 115.6  & 57.2$\pm$0.7 & 42.1$\pm$1.5 &  16.0 & 91.4$\pm$0.4 &83.5$\pm$2.5  \\\midrule
%~~- source-complex &  &   &  &  &   &  & 91.5$\pm$0.2 & \textcolor{green}{80.8$\pm$1.0} \\\midrule
\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With only reg.}}\\
% \textit{With only reg.}:  \multicolumn{9}{c|}{\cellcolor{na}}  \\
\midrule
%~~- DANN-simple &  &   &  &  &   &  & 90.2$\pm$0.5 & 71.0$\pm$3.5 \\
%~~- DANN-simple2 &  &   &  &  &   &  & 90.5$\pm$0.4 & \textcolor{blue}{87.3$\pm$0.4} \\
%~~- DANN & 60.7$\pm$0.6 & 33.9$\pm$1.1  & 220.3 & \textcolor{red}{58.6$\pm$2.6} & 42.1$\pm$0.2  & 101.7 & 90.0$\pm$0.9 & \textcolor{red}{87.0$\pm$0.6}\\
~~- Hard reg. with IG & 63.8$\pm$0.5 & 36.9$\pm$4.1  & 72.6 & \textbf{55.4$\pm$1.9} & 43.7$\pm$0.2  & 23.3 & 91.1$\pm$0.0 & 85.2$\pm$0.1  \\ %0.1, 5e-6, 0.1, 5e-6
~~- Hard reg. with SOC & 63.0$\pm$1.2 & 38.8$\pm$1.0 & 76.0 & 54.2$\pm$2.2 & 43.8$\pm$0.4  & \textbf{6.8} & 91.1$\pm$0.0 & 85.2$\pm$0.3  \\
~~- Soft reg. with IG & \textbf{63.9$\pm$1.0} & 35.3$\pm$3.2  & 182.5 & 54.7$\pm$1.4 & 42.8$\pm$1.8 & 41.6 & 91.1$\pm$0.0 & 85.0$\pm$0.2  \\ % 0.05, 5e-6, 0.1, 7e-6
~~- Soft reg. with SOC& 63.5$\pm$1.0 & \textbf{39.8$\pm$4.7}  &  \textbf{39.8} & 52.6$\pm$4.0 & \textbf{44.6$\pm$1.6}  & 7.2 & 91.1$\pm$0.0 & \textbf{85.3$\pm$0.1}  \\ \midrule

\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With reg. \& noisy labels}}\\\midrule
% \textit{With noisy labels}: &&&&&&&\\
~~- No reg.  (BabbleLabbel)   & 60.3$\pm$1.4 & 47.1$\pm$2.2  & 80.2 & 42.0$\pm$1.6 & 50.0$\pm$0.5  & 59.2 & 90.7$\pm$0.1 & 86.0$\pm$0.6  \\
~~- No reg. with soft labels (NExT)&$\pm$ & $\pm$  &  & 49.6$\pm$4.1 & 47.9$\pm$0.6 & 164.0 & 90.4$\pm$0.9 & 86.3$\pm$0.4 \\
~~- Baseline:L2-reg & 62.7$\pm$1.1 & 46.3$\pm$0.2 & 77.1 & 46.5$\pm$0.7 & 50.9$\pm$0.8  & 86.4 & 90.7$\pm$0.3 & 86.8$\pm$0.6\\
~~- Baseline:Distillation & 64.2$\pm$1.0 & $46.3\pm$0.9  & \textbf{65.4} & 46.4$\pm$1.3 & 50.4$\pm$1.1 & 49.7 & 90.6$\pm$0.5 & 86.7$\pm$1.0 \\
~~- Soft reg. with IG & \textbf{64.2$\pm$0.4} & 47.2$\pm$1.3 & 129.5 & \textbf{51.4$\pm$4.6} &  47.5$\pm$1.1  & \textbf{12.8} & \textbf{91.2$\pm$0.1} & 87.0$\pm$3.7  \\ %0.005, 7e-5, 0.02, 5e-5
~~- Soft reg. with SOC & 59.7$\pm$3.4 & \textbf{48.2$\pm$1.5}  &  207.9 & 47.4$\pm$1.9 & \textbf{51.1$\pm$1.6}  & 34.6 & 91.1$\pm$0.2 & \textbf{87.3$\pm$0.1}  \\ \midrule

Upper bound & 60.0$\pm$2.3 & 51.5$\pm$0.9  &  333.3 & 46.9$\pm$2.4 & 52.9$\pm$1.0  & 115.0  & 90.4$\pm$0.1& 92.9$\pm$0.4  \\

\bottomrule
\\
\\
\midrule
Source model (BERT-l) & 63.7$\pm$0.5 & 31.4$\pm$1.4 & 124.3 & 59.5$\pm$1.1  &  41.9$\pm$1.4  & 17.1 & 92.9$\pm$0.2 & 87.7$\pm$1.0 \\ \midrule
\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With only reg.}}\\
% \textit{With only reg.}:  \multicolumn{9}{c|}{\cellcolor{na}}  \\
\midrule
%~~- Unsupervised baseline &$\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\
%~~- Hard reg. with IG & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  \\ %0.1, 5e-6, 0.1, 5e-6
~~- Hard reg. with SOC & 64.0$\pm$1.1 & 36.6$\pm$\color{red}8.7  & 40.1 & 56.4$\pm$2.0 & 45.7$\pm$0.9  & 0.5  & 92.8$\pm$0.1 & 89.2$\pm$0.2 \\
%~~- Soft reg. with IG &  $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\ % 0.05, 5e-6, 0.1, 7e-6
~~- Soft reg. with SOC&  61.5$\pm$0.2 & 37.5$\pm$0.7  & 55.5 & 57.8$\pm$1.2 & \textcolor{red}{45.3$\pm$1.5} &  1.2 & 92.7$\pm$0.1 & \textbf{89.4$\pm$0.2}\\ \midrule

\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With reg. \& noisy labels}}\\\midrule
% \textit{With noisy labels}: &&&&&&&\\
~~- No reg. with hard labels  & 59.9$\pm$2.0 & 46.6$\pm$1.3  & 29.9 & 50.7$\pm$3.3 & 50.6$\pm$0.6  & 147.9  & 92.7$\pm$0.1  & 90.1$\pm$0.3 \\
~~- No reg. with soft labels &$\pm$ & $\pm$  &  & 55.4$\pm$0.2 & 50.0$\pm$0.4 & 75.5 & 92.6$\pm$0.1 & 89.6$\pm$0.3 \\
~~- Baseline:L2-reg. & 62.1$\pm$0.7 & 47.5$\pm$0.5  & 8.4 & 54.2$\pm$0.5 & 51.8$\pm$0.9  & 49.4 & 92.8$\pm$0.2 & 90.0$\pm$0.1 \\
~~- Baseline:Distillation & 61.0$\pm$1.3 & 46.0$\pm$2.6  & 11.1 & 48.8$\pm$1.3 & 52.6$\pm$0.4  & 81.5 & 92.7$\pm$0.1 & 89.9$\pm$0.1 \\
%~~- Soft reg. with IG &  $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\ %0.005, 7e-5, 0.02, 5e-5
~~- Soft reg. with SOC & 62.0$\pm$0.4 & \color{red}{46.1$\pm$1.0}  & 15.3 & 49.0$\pm$3.4 & \textcolor{red}{52.2$\pm$0.4}  & \textbf{10.0} & 92.7$\pm$0.2 & \textbf{90.3$\pm$0.2} \\ \midrule

Upper bound & 51.3$\pm$5.6 & 52.5$\pm$0.4  & 98.0 & 46.0$\pm$3.8 & 53.8$\pm$1.6 & 142.3 & 92.5$\pm$0.2 & 94.4$\pm$0.4 \\

\bottomrule
\\
\\
\midrule

\small Source model (RoBERTa-b) & 62.7$\pm$0.9 & 30.9$\pm$1.9  & 61.6 & $\pm$ & 39.6$\pm$1.2  &  & $\pm$ & $\pm$  \\ \midrule
\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With only reg.}}\\
% \textit{With only reg.}:  \multicolumn{9}{c|}{\cellcolor{na}}  \\
\midrule
%~~- Hard reg. with IG &  $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\ %0.1, 5e-6, 0.1, 5e-6
~~- Hard reg. with SOC &  \textbf{61.3$\pm$0.4} & \textbf{40.7$\pm$0.9}  & 39.7 & $\pm$ & 41.2$\pm$0.6  &  & $\pm$ & $\pm$ \\
%~~- Soft reg. with IG &  $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\ % 0.05, 5e-6, 0.1, 7e-6
~~- Soft reg. with SOC&  61.1$\pm$0.6 & 40.5$\pm$1.1  & \textbf{15.9} & $\pm$ & \textcolor{red}{40.9$\pm$0.6}  &  & $\pm$ & $\pm$ \\ \midrule

\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With reg. \& noisy labels}}\\\midrule
%~~- Supervised baseline & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$\\
% \textit{With noisy labels}: &&&&&&&\\
~~- No reg.  & 57.8$\pm$1.0 & 45.8$\pm$1.0 & 48.2 & $\pm$ & 48.3$\pm$2.1  &  & $\pm$ & $\pm$    \\
~~- No reg. with soft labels &$\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$ \\
~~- Baseline:L2-reg. & 57.9$\pm$3.7 & 45.5$\pm$2.4  & 26.5 & 50.4$\pm$3.3 & 49.0$\pm$2.4  & 177.6 & $\pm$ & $\pm$ \\
~~- Baseline:Distillation & 60.1$\pm$1.3 & 45.9$\pm$1.8  & 87.5 & 43.8$\pm$3.0 & 48.2$\pm$0.8  & 164.0 & $\pm$ & $\pm$ \\
%~~- Soft reg. with IG & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  &  & $\pm$ & $\pm$  \\ %0.005, 7e-5, 0.02, 5e-5
~~- Soft reg. with SOC &  57.5$\pm$0.9 & \color{red}{44.7$\pm$1.0}  & 97.8 & 48.6$\pm$1.9 & 50.1$\pm$1.7  & 77.5 & $\pm$ & $\pm$ \\ \midrule

Upper bound & 51.4$\pm$3.2 & 50.6$\pm$0.4 & 263.2 & 52.2$\pm$4.9 & 50.5$\pm$1.5  & 294.0 & $\pm$ & $\pm$ \\

\bottomrule

\end{tabular}
}
\label{tab:main_results_new}
\vspace{-0.5cm}
\end{table*}

==> floats/tab_main_new.tex <==


\begin{table*}[t]
% \vspace{-0.1cm}
\centering
\caption{\textbf{Main Results on BERT-base for different regularization settings on three pairs of datasets.} We report F1 scores on source domain and target domain, and FPRD on IPTTS as fairness metric for hate speech task. Best results are \textbf{bold}. 
%Regularization based on both hard- and soft-matching improves the target domain performance of the source model, and also reduces unintended bias.
}
\vspace{-0.2cm}
\scalebox{0.70}{
\begin{tabular}{@{}l|ccc|ccc|cc@{}}
\toprule
\textbf{Dataset} & \multicolumn{3}{c|}{\small\textbf{HatEval $\rightarrow$ GHC}} & \multicolumn{3}{c|}{\small\textbf{Stormfront $\rightarrow$ GHC}} & \multicolumn{2}{c}{\small\textbf{AmazonMusic $\rightarrow$ SST-2}} \\ \midrule
\textbf{Metrics}           & 
\textbf{\small\begin{tabular}[c]{@{}c@{}}Source  F1 ($\uparrow$)\end{tabular}} & \textbf{\small\begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} & 
\textbf{\small\begin{tabular}[c]{@{}c@{}}Source F1($\uparrow$)\end{tabular}} &
\textbf{\small\begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} & \textbf{\small\begin{tabular}[c]{@{}c@{}}Source F1 ($\uparrow$)\end{tabular}} &  \textbf{\small \begin{tabular}[c]{@{}c@{}}Target F1 ($\uparrow$)\end{tabular}} \\ \midrule
Source model & 64.2$\pm$0.3 & 29.5$\pm$2.5  & 115.6  & 57.2$\pm$0.7 & 42.1$\pm$1.5 &  16.0 & 91.4$\pm$0.4 &83.5$\pm$2.5  \\ \midrule
\multicolumn{9}{l}{\cellcolor{na}\hspace{-0.2cm}\textit{With only reg.}}\\
% \textit{With only reg.}:  \multicolumn{9}{c|}{\cellcolor{na}}  \\
\midrule
~~- Hard reg. with IG & 63.2$\pm$0.6 & 34.4$\pm$1.4  & 197.2 & \textbf{55.4$\pm$1.9} & 43.7$\pm$0.2  & 23.3 & 91.1$\pm$0.0 & 85.2$\pm$0.1  \\ %0.1, 5e-6, 0.1, 5e-6
~~- Hard reg. with SOC & 63.1$\pm$0.4 & 37.6$\pm$2.6  & 73.6 & 54.2$\pm$2.2 & 43.8$\pm$0.4  & \textbf{6.8} & 91.1$\pm$0.0 & 85.2$\pm$0.3  \\
~~- Soft reg. with IG & \textbf{63.2$\pm$0.3} & 33.2$\pm$0.8  & 204.9  & 54.7$\pm$1.4 & 42.8$\pm$1.8 & 41.6 & 91.1$\pm$0.0 & 85.0$\pm$0.2  \\ % 0.05, 5e-6, 0.1, 7e-6
~~- Soft reg. with SOC& 63.2$\pm$1.1 & \textbf{39.5$\pm$1.5}  & \textbf{19.4}  & 52.6$\pm$4.0 & \textbf{44.6$\pm$1.6}  & 7.2 & 91.1$\pm$0.0 & \textbf{85.3$\pm$0.1}  \\ \midrule

\multicolumn{9}{l}{\hspace{-0.2cm}\textit{With reg. \& noisy labels} \cellcolor{na}}\\\midrule
% \textit{With noisy labels}: &&&&&&&\\
~~- No reg.    & 56.3$\pm$0.8 & \textbf{48.7$\pm$1.4}  & 148.0 & 42.0$\pm$1.6 & 50.0$\pm$0.5  & 59.2 & 90.7$\pm$0.1 & 86.0$\pm$0.6  \\
~~- Soft reg. with IG & \textbf{61.9$\pm$0.9} & 48.1$\pm$3.0 & 199.4  & \textbf{51.4$\pm$4.6} &  47.5$\pm$1.1  & \textbf{12.8} & \textbf{91.2$\pm$0.1} & 87.0$\pm$3.7  \\ %0.005, 7e-5, 0.02, 5e-5
~~- Soft reg. with SOC & 60.0$\pm$2.3 & 48.1$\pm$0.7  & \textbf{105.7} & 47.4$\pm$1.9 & \textbf{51.1$\pm$1.6}  & 34.6 & 91.1$\pm$0.2 & \textbf{87.3$\pm$0.1}  \\ \midrule

Upper bound & 60.0$\pm$2.3 & 51.5$\pm$0.9  &  333.3 & 46.9$\pm$2.4 & 52.9$\pm$1.0  & 115.0  & 90.4$\pm$0.1& 92.9$\pm$0.4  \\

 \bottomrule
\end{tabular}
}
\label{tab:main_results_new}
\vspace{-0.5cm}
\end{table*}

==> floats/tab_nonhate_new.tex <==
\begin{table}[h]
\vspace{-0.1cm}
\centering
\caption{\textbf{Ablation study on hate-labeled and nonhate-labeled rules on Gab Hate Corpus.} Hate-labeled rules contain more precise information to better improve model performance.}
\vskip 0.15in
\scalebox{0.75}{
\begin{tabular}{@{}lcccc}
\toprule
\textbf{Dataset} & \multicolumn{2}{c}{\small\textbf{\begin{tabular}[c]{@{}c@{}}Stormfront$\rightarrow$GHC\end{tabular}}} & \multicolumn{2}{c}{\small\textbf{\begin{tabular}[c]{@{}c@{}}Hateval$\rightarrow$GHC\end{tabular} }} \\ 
\midrule
\textbf{Metrics}           & \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} &   \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}} FPRD ($\downarrow$)\end{tabular}} \\ \midrule
\textbf{Source Model} & 42.1$\pm$1.5 &  16.0  & 29.5$\pm$2.5 & 115.6 \\
\textbf{Nonhate-labeled rules} & 43.2$\pm$0.4 &  9.0  & 32.1$\pm$0.5 & 175.3 \\
\textbf{All rules} & 43.2$\pm$0.4 & 8.2  &  32.4$\pm$0.2  & 174.5 \\
\textbf{Hate-labeled rules} & \textbf{44.6$\pm$1.6}  &  \textbf{7.2} & \textbf{39.5$\pm$1.5} & \textbf{19.0} \\
 \bottomrule
\end{tabular}
}
\label{tab:ablation_nonhate_rules_new}
% \vspace{-0.2cm}
\end{table}

==> floats/tab_nonhate_rules.tex <==
\begin{table}[h]
\centering
\caption{Studying effects of hateful and non-hateful rules on Gab Hate Corpus.}
\vskip 0.15in
\scalebox{0.7}{
\begin{tabular}{@{}l|cc|cc}
\toprule
\textbf{Dataset} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Stormfront\\ $\rightarrow$ GHC\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Hateval\\ $\rightarrow$ GHC\end{tabular} }} \\ \midrule
\textbf{Metrics}           & \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} &   \textbf{\begin{tabular}[c]{@{}c@{}}F1 ($\uparrow$)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} \\ \midrule
\textbf{Original Model} & 42.1$\pm$1.5 &  16.0  & 29.5$\pm$2.5 & 115.6 \\
\textbf{Nonhate-labeled rules} & 43.4$\pm$0.4 &  9.0  & 32.1$\pm$0.5 & 175.3 \\
\textbf{All rules} & 45.0$\pm$0.8 &  9.0  &  32.9$\pm$0.6  & 183.4 \\
\textbf{Hate-labeled rules} & 45.7$\pm$1.4 &  12.6  & 39.9$\pm$2.1 & 50.2 \\
 \bottomrule
\end{tabular}
}
\label{tab:ablation_nonhate_rules}
\vspace{-0.2cm}
\end{table}

==> floats/tab_sensitivity_ghc.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Method  & F1 & IPTT F1 & IPTT FPR\\
\midrule
\makecell[l]{Original model\\from Stormfront} & $0.421\pm0.015$ & $0.529\pm0.099$ & $0.013\pm0.006$\\
Sampling 2000 & &  &   \\
Sampling 3381 & & & \\
Non-hate rules & & & \\
\midrule
\makecell[l]{Original model\\from HatEval} & $0.295\pm0.025$ &$0.332\pm0.153$ &$0.053\pm0.049$\\
% Soft match reg. importance & $0.361\pm0.011$ & $0.436\pm0.011$ & $0.395\pm0.003$\\
Sampling 2000 & &  &   \\
Sampling 3381 & & & \\
Non-hate rules & & & \\
\bottomrule
\end{tabular}
}
\vspace{-0.2cm}

\caption{Studying sensitivity of different negative sampling on Gab Hate Corpus.}
\label{sensitivity-negative-sampling-table}
\end{table}


==> floats/tab_sst2.tex <==
\begin{table*}[t]
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccr}
\toprule
Method  & Precision & Recall & F1\\
\midrule
Original model from AmazonMusic & $0.902\pm0.032$ & $0.781\pm0.064$ & $0.835\pm0.025$\\
Only Reg: Hard match reg. with IG & $0.868\pm0.001$ & $0.836\pm0.002$ & $0.852\pm0.001$ \\ % reg=0.1, lr=5e-6
%Only Reg: Hard match reg. with IG, nointer & $0.867 \pm0.003$ & $0.838\pm0.004$ & $0.852\pm0.001$ \\ % reg=0.1, lr=5e-6
Only Reg: Hard match reg. with SOC & $0.867\pm0.003$ & $0.837\pm0.007$ & $0.852\pm0.003$\\
Only Reg: Soft match reg. with IG & $0.867\pm0.002$ & $0.834\pm0.006$ & \textcolor{red}{$0.850\pm0.002$} \\ % reg=0.01, lr=5e-6
%Only Reg: Soft match reg. with IG, nointer & $0.862\pm0.011$ & $0.840\pm0.015$ & $0.851\pm0.003$ \\ % reg=0.1, lr=8e-6

Only Reg: Soft match reg. with SOC & $0.863\pm0.007$ & $0.843\pm0.008$ & $0.853\pm0.001$\\\midrule
Only Labels: Hard match label & $0.846\pm0.005$ & $0.874\pm0.016$ & $0.860\pm0.006$ \\
%Reg + Label: Hard match label + Neg Samples + Soft match reg. with LIME & & & & \\ % Mean
Reg + Label: Hard match label + Soft match reg. with IG & $ 0.873 \pm 0.004$  &  $0.877 \pm 0.030 $ &  $0.870 \pm 0.037 $\\ % 0.05, 5e-6
%Reg. + Labels: Hard match label + Soft match reg. with IG, nointer  & $0.871 \pm 0.003 $  & $0.851 \pm 0.019 $ & $0.892 \pm 0.015$ & \\ % 0.01, 8e-6
Reg. + Labels: Hard match label + Soft match reg. with SOC &  $0.866\pm0.003$ & $0.880\pm0.005$ & $0.873\pm0.001$ \\ % Mean
Fine-tune with SST-2 (Upper bound) & $0.909\pm0.009$& $0.949\pm0.004$& $0.929\pm0.004$\\

\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\caption{Precision, recall and F1 score for different regularization settings on sentiment analysis task.}
\label{sst-main-table}
\end{table*}

